ToonTalker: Cross-Domain Face Reenactment

We target cross-domain face reenactment in this paper, i.e., driving a cartoon image with the video of a real person and vice versa. Recently, many works have focused on one-shot talking face generation to drive a portrait with a real video, i.e., within-domain reenactment. Straightforwardly applying those methods to cross-domain animation will cause inaccurate expression transfer, blur effects, and even apparent artifacts due to the domain shift between cartoon and real faces. Only a few works attempt to settle cross-domain face reenactment. The most related work AnimeCeleb requires constructing a dataset with pose vector and cartoon image pairs by animating 3D characters, which makes it inapplicable anymore if no paired data is available. In this paper, we propose a novel method for cross-domain reenactment without paired data. Specifically, we propose a transformer-based framework to align the motions from different domains into a common latent space where motion transfer is conducted via latent code addition. Two domain-specific motion encoders and two learnable motion base memories are used to capture domain properties. A source query transformer and a driving one are exploited to project domain-specific motion to the canonical space. The edited motion is projected back to the domain of the source with a transformer. Moreover, since no paired data is provided, we propose a novel cross-domain training scheme using data from two domains with the designed analogy constraint. Besides, we contribute a cartoon dataset in Disney style. Extensive evaluations demonstrate the superiority of our method over competing methods.

==> fig_tex/fig_ablation_data.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{asset/ablation_data.pdf}
\caption{Comparison with training on the mixed data.}
\label{fig:ablation_data}
\end{figure}


==> fig_tex/fig_cartoon_model.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{asset/cartoon_model.pdf}
\caption{Comparison with only using cartoon domain model.}
\label{fig:cartoon_model}
\end{figure}

==> fig_tex/fig_codeloss.tex <==
\begin{figure*}[htb]
\centering
\includegraphics[width=\linewidth]{asset/ablation.pdf}
\caption{Qualitative ablation studies.}
\label{fig:codeloss}
\end{figure*}


==> fig_tex/fig_real_model.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{asset/real_model.pdf}
\caption{Comparison with only using real domain model.}
\label{fig:real_model}
\end{figure}
